Scalar auxiliary variable (SAV) stabilization of implicit-explicit (IMEX) time integration schemes for nonlinear structural dynamics

Implicit-explicit (IMEX) time integration schemes are well suited for nonlinear structural dynamics because of their low computational cost and high accuracy. However, stability of IMEX schemes cannot be guaranteed for general nonlinear problems. In this article, we present a scalar auxiliary variable (SAV) stabilization of high-order IMEX time integration schemes that leads to unconditional stability. The proposed IMEX-BDFk-SAV schemes treat linear terms implicitly using kth-order backward difference formulas (BDFk) and nonlinear terms explicitly. This eliminates the need for iterations in nonlinear problems and leads to low computational cost. Truncation error analysis of the proposed IMEX-BDFk-SAV schemes confirms that up to kth-order accuracy can be achieved and this is verified through a series of convergence tests. Unlike existing SAV schemes for first-order ordinary differential equations (ODEs), we introduce a novel SAV for the proposed schemes that allows direct solution of the second-order ODEs without transforming them to a system of first-order ODEs. Finally, we demonstrate the performance of the proposed schemes by solving several nonlinear problems in structural dynamics and show that the proposed schemes can achieve high accuracy at a low computational cost while maintaining unconditional stability.

==> temp.tex <==
\subsection{Basic equations}
For the linear elastic material without viscous damping, the equilibrium equation of the standard finite element democratization is 
\begin{equation}
    \mathbf{M} \mathbf{a}(t) + \mathbf{K}\mathbf{d}(t)= \mathbf{f} (t)
    \label{eqn:GovEqn}
\end{equation}
where $\mathbf{M}$, $\mathbf{K}$, $\mathbf{a}$, $\mathbf{d}$, and $\mathbf{f}$ denote the global mass, stiffness matrices, acceleration, displacement, and external force vectors, respectively. Given the known solutions at time $t_n$ with time step size $\Delta t$, the solutions at the next time step $t_{n+1}=t_{n}+\Delta t$ can be calculated using the time integration scheme.

Using the Bathe implicit scheme, for which the two sub-steps are used, we can obtained the transient solutions for the governing equation: 
\begin{align} 
    &\textrm{First sub-step:} & \mathbf{M} \mathbf{a}_{n+\gamma} + \mathbf{K}\mathbf{d}_{n+\gamma}= \mathbf{f}_{n+\gamma}  \nonumber \\
    &&\mathbf{v}_{n+\gamma} = \mathbf{v}_{n} + \frac{\gamma\Delta t}{2}(\mathbf{a}_{n} + \mathbf{a}_{n+\gamma})  \nonumber \\
    &&\mathbf{d}_{n+\gamma} = \mathbf{d}_{n} + \frac{\gamma\Delta t}{2}(\mathbf{v}_{n} + \mathbf{v}_{n+\gamma}) \nonumber \\
    &\textrm{Second sub-step:} &\mathbf{M} \mathbf{a}_{n+1} + \mathbf{K}\mathbf{d}_{n+1}= \mathbf{f}_{n+1}  \nonumber \\
    &&\mathbf{v}_{n+1} = \mathbf{v}_{n} + \Delta t(s_0 \mathbf{a}_n + s_1 \mathbf{a}_{n+\gamma} + s_2 \mathbf{a}_{n+1} )  \nonumber \\
    &&\mathbf{d}_{n+1} = \mathbf{d}_{n} + \Delta t(q_0 \mathbf{v}_n + q_1 \mathbf{v}_{n+\gamma} + q_2 \mathbf{v}_{n+1} ) \label{eqn:Bathe}
\end{align}
where $\mathbf{v}$ and $\gamma$ are the velocity vector and the splitting ratio, respectively. $s_0$, $s_1$, $s_2$, $q_0$, $q_1$, and $q_2$ are Bathe parameters depending on the Bathe schemes:
\begin{align}
    &\gamma\textrm{-Bathe:} &s_0=q_0=s_1=q_1=\frac{1}{4-2\gamma}; \quad s_2=q_2=\frac{1-\gamma}{2-\gamma} \nonumber \\
    &\rho_\infty\textrm{-Bathe:} &s_1=q_1=\frac{\rho_\infty+1}{2\gamma(\rho_\infty-1)+4}; \nonumber \\
    &&s_0=q_0=(\gamma-1)q_1+\frac{1}{2}; \quad  s_2=q_2=-\gamma q_1+\frac{1}{2} \nonumber \\
    &\beta_1/\beta_2\textrm{-Bathe:} &s_0=q_0=\gamma(1-\beta_1); \nonumber \\
    &&s_1=q_1=\gamma(\beta_1+\beta_2-1)+1-\beta_2; \quad s_2=q_2=(1-\gamma)\beta_2 \label{eqn:Bathepara}
\end{align}

Note that the $\gamma$-Bathe scheme is identical to the $\rho_\infty$-Bathe scheme with $\rho_\infty=0$. In Ref.~\cite{malakiyeh2019bathe}, they have used $\beta_2=1-\beta_1$ and $\beta_2=2\beta_1$ with $\gamma=0.5$. we recall that the $\beta_1/\beta_2$-Bathe schemes with $\beta_2=2\beta_1$ and $\beta_2=1-\beta_1$ are first- and second-order accurate, respectively. Moreover, the $\beta_1/\beta_2$-Bathe scheme with $\beta_2=1-\beta_1$ gives the same characteristics as the $\rho_\infty$-Bathe scheme. Therefore, in this paper, we refer to the $\beta_1/\beta_2$-Bathe scheme with $\beta_2=2\beta_1$ and $\gamma=0.5$ as the first-order $\beta_1/\beta_2$-Bathe scheme.


\subsection{Energy method}
In this section, the energy formulation for the Bathe scheme is derived by using the modal approach: $\mathbf{M}\rightarrow 1;\,\mathbf{K}\rightarrow \omega^2;\,\mathbf{a}\rightarrow a;\,\mathbf{v}\rightarrow v;\,\mathbf{d}\rightarrow d;$ and $\,\mathbf{f}\rightarrow r$ (here, $\omega$ is the natural frequency).

From Eq.~(\ref{eqn:Bathe}) with the $\rho_\infty$-Bathe scheme in Eq.~(\ref{eqn:Bathepara}), one obtains
\begin{align}
    \Delta T(a) + \Delta V(v) + D(a, v) = E_{ext}(a,v,r)
\end{align}
where $\Delta T$, $\Delta V$, $\Delta D$, and $\Delta E_{ext}$ are the energy variation terms related to the kinetic energy, strain energy, numerical damping, and external force, respectively:
\begin{align}
    & \Delta T(a) = (a_{n+1}^2-a_n^2)/2; \quad \Delta V(v) = (v_{n+1}^2-v_n^2)\omega^2/2;
    \nonumber \\
    & \Delta D(a, v) =  \frac{(1-\rho_\infty^2)\gamma^2(1-\gamma)^2\Delta t^2\omega^2 \left\{\Delta a^2+\Delta v^2 \omega ^2\right\}}{8(2-\gamma(1-\rho_\infty))^2+2(1-\rho_\infty)^2\gamma^2(1-\gamma)^2\Delta t^2 \omega^2};
    \nonumber \\
    & \Delta E_{ext}(a,v,r) =\begin{matrix} \frac{1}{\Delta t}\Delta v \Delta r \\ + \frac{(1+\rho_\infty)\left\{ 2(2-\gamma(1-\rho_\infty))\Delta a+(1-\rho_\infty)\gamma(1-\gamma)\Delta t\omega^2\Delta v \right\}}{4(2-\gamma(1-\rho_\infty))^2+(1-\rho_\infty)^2\gamma^2(1-\gamma)^2\Delta t^2 \omega^2}(\gamma r_{n+1} -r_{n+\gamma} + (1-\gamma)r_n) \end{matrix}
\end{align}

Since the term related to the external force has no impact on the stability of the time integration scheme \cite{liu1982mixed}, $D(\Delta a, \Delta v) \ge 0$ in order to have stability characteristics. Therefore, the stability condition is $-1 \le \rho_\infty \le 1$ for all values of $\gamma$ to have unconditionally stability, which is identical to the stability criteria from spectral radius of the amplification matrix \cite{noh2019bathe}.

For the first-order $\beta_1/\beta_2$-Bathe scheme with $\gamma=0.5$, the energy derivations are
\begin{align}
    & \Delta T(a) = (a_{n+1}^2-a_n^2)/2; \quad \Delta V(v) = (v_{n+1}^2-v_n^2)\omega^2/2;
    \nonumber \\
    & \Delta D(a, v) =  \frac{(4(3\beta_1-1)+0.5\beta_1^2\Delta t^2 \omega_0^2) \left\{\Delta a^2+\Delta v^2 \omega ^2\right\}}{16+\beta_1^2\Delta t^2 \omega^2};
    \nonumber \\
    & \Delta E_{ext}(a,v,r) = \frac{1}{\Delta t}\Delta v \Delta r + \frac{(1-\beta_1)\left\{ 4\Delta a+\beta_1\Delta t\omega^2\Delta v \right\}}{16+\beta_1^2 \Delta t^2 \omega^2}(r_{n+1} -2r_{n+0.5} + r_n)
\end{align}

Therefore, $\beta_1 \ge 1/3$ is the unconditionally stability condition, which is identical to the stability condition obtained from spectral radius \cite{kwon2020analysis}.

Since the interface energy for the MTS methods is derived from the energy variations of the external force \cite{gravouil2001multi,combescure2002numerical,prakash2004feti}, we only focus on the external force energy variations.

Considering all $n$ natural frequencies, the external energy variation of the first-order $\beta_1/\beta_2$-Bathe scheme with $\gamma=0.5$ is
\begin{align}
     &\Delta E_{ext} = \frac{1}{\Delta t}\Delta \mathbf{v}_{mode}^T \Delta \mathbf{f}_{mode} \nonumber \\ 
     & + (1-\beta_1)\left( 4\Delta \mathbf{a}_{mode}^T+\beta_1\Delta t\Delta \mathbf{v}_{mode}^T \boldsymbol{\Lambda}^T \right)\left(16\mathbf{I}+\beta_1^2 \Delta t^2 \boldsymbol{\Lambda}\right)^{-T}\left( \mathbf{f}_{mode,n+1} -2\mathbf{f}_{mode,n+0.5} + \mathbf{f}_{mode,n}\right)
\end{align}
where $\mathbf{v}_{mode}$, $\mathbf{a}_{mode}$, and $\mathbf{f}_{mode}$ are the vectors of all modal degrees of freedom for $v$, $a$, and $r$, respectively. $\boldsymbol{\Lambda}$ is a diagonal matrix of the eigenvalues ($=\textrm{diag}(\omega_1^2,\omega_2^2,...,\omega_n^2)$), here $\omega_i$ is the $i$-th natrual frequency component. Using the eigenvectors $\mathbf{x}$ of the problem $\mathbf{K}\mathbf{x}=\mathbf{M}\mathbf{x}\boldsymbol{\Lambda}$,
\begin{align}
     &\Delta E_{ext}(\mathbf{a},\mathbf{v},\mathbf{f}) = \frac{1}{\Delta t}\Delta \mathbf{v}^T \Delta \mathbf{f} \nonumber \\ 
     & + (1-\beta_1)\left( 4\Delta \mathbf{a}^T \mathbf{M}^T +\beta_1\Delta t\Delta \mathbf{v}^T \mathbf{K}^T \right)\left(16\mathbf{M}+\beta_1^2 \Delta t^2 \mathbf{K}\right)^{-T}\left( \mathbf{f}_{n+1} -2\mathbf{f}_{n+0.5} + \mathbf{f}_{n}\right) \label{eqn:ExtEnergy_beta}
\end{align}

Similar to the $\beta_1/\beta_2$-Bathe scheme, the external energy variation for the $\rho_\infty$-Bathe scheme can be expressed by
\begin{align}
     &\Delta E_{ext}(\mathbf{a},\mathbf{v},\mathbf{f}) = \frac{1}{\Delta t}\Delta \mathbf{v}^T \Delta \mathbf{f} \nonumber \\&+ (1+\rho_\infty) \left( \begin{matrix} 2(2-\gamma(1-\rho_\infty))\Delta \mathbf{a}^T\mathbf{M}^T \\ +(1-\rho_\infty)\gamma(1-\gamma)\Delta t\Delta \mathbf{v}^T \mathbf{K}^T \end{matrix} \right) \left( \begin{matrix} 4(2-\gamma(1-\rho_\infty))^2\mathbf{M} \\ +(1-\rho_\infty)^2\gamma^2(1-\gamma)^2\Delta t^2 \mathbf{K} \end{matrix} \right)^{-T} \left( \begin{matrix}\gamma \mathbf{f}_{n+1} -\mathbf{f}_{n+\gamma}  \\+ (1-\gamma)\mathbf{f}_n \end{matrix} \right) \label{eqn:ExtEnergy_rho}
\end{align}
